SAGE -- A Tool for Optimal Deployments in Kubernetes Clusters

Cloud computing has brought a fundamental transformation in how organizations operate their applications, enabling them to achieve affordable high availability of services. Kubernetes has emerged as the preferred choice for container orchestration and service management across many Cloud computing platforms. The scheduler in Kubernetes plays a crucial role in determining the placement of newly deployed service containers. However, the default scheduler, while fast, often lacks optimization, leading to inefficient service placement or even deployment failures. This paper introduces SAGE, a tool for optimal solutions in Kubernetes clusters that can also assist the Kubernetes default scheduler and any other custom scheduler in application deployment. SAGE computes an optimal deployment plan based on the constraints of the application to be deployed and the available Cloud resources. We show the potential benefits of using SAGE by considering test cases with various characteristics. It turns out that SAGE surpasses other schedulers by comprehensively analyzing the application demand and cluster image. This ability allows it to better understand the needs of the pods, resulting in consistently optimal solutions across all scenarios. The accompanying material of this paper is publicly available at https://github.com/SAGE-Project/SAGE-Predeployer.

==> NewCaseStudies.tex <==
\section{Additional Case Studies} \label{sec:NewCaseStudies}
\subsection{Wordpress}\label{sec:Wordpress}
\emph{Wordpress}, an open-source application which is frequently used in creating websites, blogs and applications (Figure~\ref{fig:Wordpress}). 
\begin{figure}[h!]
	\centering
	\includegraphics[width=0.45\textwidth]{Wordpress.png}
	\caption{Wordpress Application}
	\label{fig:Wordpress}
\end{figure}
The two important characteristics of Wordpress, namely high-load and fault tolerant are ensured by load balancing. One possibility is to balance load at the DNS level using servers like Bind\footnote{\url{https://www.isc.org/downloads/bind/}}: multiple DNS requests to resolve the website name will result in different IPs from a given pool of machines, on each of which a separate Wordpress instance is running. Alternatively one can use as website entry point an HTTP reverse proxy capable of load balancing (and caching, for added benefit) such as Varnish. In both cases, Wordpress instances will need to be configured to connect to the same MySQL database, to avoid delivering inconsistent results to users. Also, having redundancy and balancing at the front-end level, one usually expects to have them also at the Database Management System (DBMS) level. One way to achieve that is to use a MySQL cluster, and configure the Wordpress instances with multiple entry points to it. In the deployment scenario considered by us, the following constraints must be fulfilled:
\begin{inparaenum}[\itshape (i)\upshape]
	\item DNSLoadBalancer requires at least one instance of Wordpress and DNSLoadBalancer can serve at most 7 Wordpress instances (\emph{Require-Provide} constraint).
	%$$\sum_{k=1}^{M}a_{3 k} \le 7\sum_{k=1}^{M}a_{1 k}, \quad k=\overline{1,M}$$
	\item HTTPLoadBalancer requires at least one Wordpress instance and HTTPLoadBalancer can serve at most 3 Wordpress instances (\emph{Require-Provide} constraint).
	%$$\sum_{k=1}^{M}a_{4 k} \le 3\sum_{k=1}^{M}a_{1 k}, \quad k=\overline{1,M}$$
	\item Wordpress requires at least 2 instances of MySQL and MySQL can serve at most 3 Wordpress (\emph{\textbf{Require-Provide}} constraint).
	%$$3 \sum_{k=1}^{M}a_{1 k} \le2\sum_{k=1}^{M}a_{2 k}, \quad k=\overline{1,M}$$
	\item Only one type of Balancer must be deployed (\emph{Exclusive deployment} constraint).
	%$$ H(\sum_{k=1}^{M} a_{3k}) + H (\sum_{k=1}^{M} a_{4k}) + H (\sum_{k=1}^{M} a_{5k} ) = 1
	%$$
	%$$\left(\sum_{k=1}^{M}\!a_{ik}\! = \!0 \!\lor \!\sum_{k=1}^{M}\!a_{ik} \!\ge\! 1\! \right) \land \sum_{k=1}^{M}\left(a_{3k} \!+ \!a_{4k}\right) \!\ge 1, \quad i \!\in \!\{3,4\}, \quad k=\overline{1,M}
	%$$
	%$$\left(\sum_{k=1}^{M}\!a_{ik}\! = \!0 \!\lor \!\sum_{k=1}^{M}\!a_{ik} \!\ge\! 1\! \right) \land \sum_{k=1}^{M}\left(a_{3k} \!+ \!a_{5k}\right) \!\ge 1, \quad i \!\in \!\{3,5\}, \quad k=\overline{1,M}
	%$$
	\item Since Varnish exhibits load balancing features, it should not be deployed on the same VM as with another type of Balancer (\emph{Conflict} constraint). Moreover, Varnish and MySQL should not be deployed on the same VM because it is best practice to isolate the DBMS level of an application (\emph{\textbf{Conflict}} constraint).
	%$$a_{5 k} + a_{i k} \leq 1, \quad i \in \{2, 3, 4\}, \quad k=\overline{1,M} $$
	\item At least 2 instances of Varnish must be deployed too  (\emph{\textbf{Deployment with bounded number of instances}} constraint, in particular \emph{\textbf{lower bound}}).
	%$$\sum_{k=1}^{M}a_{5k} \ge 2$$
	\item At least 2 different entry points to the MySQL cluster (\emph{\textbf{Deployment with bounded number of instance}} constraint, in particular \emph{\textbf{lower bound}}).
	%$$\sum_{k=1}^{M}a_{2kx} \ge 2$$
	\item No more than 1 DNS server deployed in the administrative domain (\emph{\textbf{Deployment with bounded number of instances}} constraint, in particular \emph{\textbf{upper bound}}).
	%$$\sum_{k=1}^{M}a_{3k} \le 1$$
	\item Balancer components must be placed on a single VM, so they are considered to be in \emph{\textbf{conflict}} with all the other components.
	%	\begin{align*}
	%	& a_{3 k} + a_{i k} \leq 1 \quad i \in \{1, 2, 5\}\\
	%	& a_{4 k} + a_{i k} \leq 1 \quad i \in \{1, 2, 5\} \\
	%	\end{align*}
\end{inparaenum}

Wordpress instances can be scaled up and down based on the requests. Here, we consider the scenarios when Wordpress has 3, respectively 8 instances. 

In order to deploy the application, SAGE proceeds as follows:
\begin{itemize}
	\item SAGE Recommendation Engine is called which, given Wordpress description (JSON file) it outputs the arrangement of component instances on available resources (assignment matrix), the type of resources and the minimal price as a JSON file.
	\item Next SAGE Predeployer is called which ...
\end{itemize}

In case of deploying Wordpress with 3, respectively 8 instances, SAGE Recommendation Engine outputs the assignment matrix two types deployment configurations, one which uses the DNS Load Balancer, the other HTTP Load Balancer (see Tables \ref{tab:Wordpress3SAGE} and \ref{tab:Wordpress8SAGE}).
\begin{table}[h!]
	\centering
	\begin{tabular}{|l||*{5}{c|}}\hline
		\backslashbox{Pod}{Node}
		&\makebox[2em]{N1}&\makebox[1em]{N2}&\makebox[1em]{N3}&\makebox[1em]{N4}&\makebox[1em]{N5}\\\hline\hline
		WordPress &   1    &                 &            1     &           1      &\\\hline
		MySQL     &   1    &    1            &                  &     &\\\hline
		DNS       &        &                 &                  &     & 1\\\hline
		HTTP      &&&&&\\\hline
		Varnish   &        &                 &             1     &    1 &\\\hline
	\end{tabular}
	\caption{Optimal placement of pods for Wordpress application with 3 Wordpress instances by SAGE}
	\label{tab:Wordpress3SAGE}
\end{table}

\begin{table}[h!]
	\centering
	\begin{tabular}{|l||*{9}{c|}}\hline
		\backslashbox{Pod}{Node}
		&\makebox[2em]{N1}&\makebox[1em]{N2}&\makebox[1em]{N3}&\makebox[1em]{N4}&\makebox[1em]{N5}&\makebox[1em]{N6}&\makebox[1em]{N7}&\makebox[1em]{N8}&\makebox[1em]{N9}\\\hline\hline
		WordPress &   1    & 1               &            1     &           1      & 1 &1 &1 &  & 1\\\hline
		MySQL     &   1    &                 &            1     &           1      & 1 & & & 1 &\\\hline
		DNS       &   1    &                 &            1     &           1      & 1 & & & 1 &\\\hline
		HTTP      &   1    &                 &            1     &           1      & 1 & & & ? &\\\hline
		Varnish &   1    &                 &            1     &           1      & 1 & & & &\\\hline
	\end{tabular}
	\caption{TODO: Optimal placement of pods for Wordpress application with 8 Wordpress instances by SAGE}
	\label{tab:Wordpress8SAGE}
\end{table}

We used the number of nodes and their characteristics for testing Boreas and K8s. Boreas was able to deploy all instances on these nods on both cases, while K8s failed to deploy the DNS load balancer for Wordpress3, respectivelly the HTTP load balancer for Wordpress8. Explanation???


\subsection{Wordpress Application}
\emph{Wordpress} open-source application is frequently used in creating websites, blogs and applications. We chose it in order to compare our approach to Zephyrus and Zephyrus2 deployment tools~\cite{DBLP:conf/kbse/CosmoLTZZEA14,DBLP:conf/setta/AbrahamCJKM16}. In \cite{DBLP:conf/kbse/CosmoLTZZEA14,DBLP:conf/setta/AbrahamCJKM16}, the authors present a high-load and fault tolerant Wordpress (Figure~\ref{fig:Wordpress}) deployment scenario. The two characteristics are ensured by load balancing. One possibility is to balance load at the DNS level using servers like Bind\footnote{\url{https://www.isc.org/downloads/bind/}}: multiple DNS requests to resolve the website name will result in different IPs from a given pool of machines, on each of which a separate Wordpress instance is running. Alternatively one can use as website entry point an HTTP reverse proxy capable of load balancing (and caching, for added benefit) such as Varnish. In both cases, Wordpress instances will need to be configured to connect to the same MySQL database, to avoid delivering inconsistent results to users. Also, having redundancy and balancing at the front-end level, one usually expects to have them also at the Database Management System (DBMS) level. One way to achieve that is to use a MySQL cluster, and configure the Wordpress instances with multiple entry points to it. In the deployment scenario considered by us, the following constraints must be fulfilled:
\begin{inparaenum}[\itshape (i)\upshape]
	\item DNSLoadBalancer requires at least one instance of Wordpress and DNSLoadBalancer can serve at most 7 Wordpress instances (\emph{\textbf{Require-Provide}} constraint).
	%$$\sum_{k=1}^{M}a_{3 k} \le 7\sum_{k=1}^{M}a_{1 k}, \quad k=\overline{1,M}$$
	\item HTTPLoadBalancer requires at least one Wordpress instance and HTTPLoadBalancer can serve at most 3 Wordpress instances (\emph{\textbf{Require-Provide}} constraint).
	%$$\sum_{k=1}^{M}a_{4 k} \le 3\sum_{k=1}^{M}a_{1 k}, \quad k=\overline{1,M}$$
	\item Wordpress requires at least 2 instances of MySQL and MySQL can serve at most 3 Wordpress (\emph{\textbf{\textbf{Require-Provide}}} constraint).
	%$$3 \sum_{k=1}^{M}a_{1 k} \le2\sum_{k=1}^{M}a_{2 k}, \quad k=\overline{1,M}$$
	\item Only one type of Balancer must be deployed (\emph{\textbf{Exclusive deployment}} constraint).
	%$$ H(\sum_{k=1}^{M} a_{3k}) + H (\sum_{k=1}^{M} a_{4k}) + H (\sum_{k=1}^{M} a_{5k} ) = 1
	%$$
	%$$\left(\sum_{k=1}^{M}\!a_{ik}\! = \!0 \!\lor \!\sum_{k=1}^{M}\!a_{ik} \!\ge\! 1\! \right) \land \sum_{k=1}^{M}\left(a_{3k} \!+ \!a_{4k}\right) \!\ge 1, \quad i \!\in \!\{3,4\}, \quad k=\overline{1,M}
	%$$
	%$$\left(\sum_{k=1}^{M}\!a_{ik}\! = \!0 \!\lor \!\sum_{k=1}^{M}\!a_{ik} \!\ge\! 1\! \right) \land \sum_{k=1}^{M}\left(a_{3k} \!+ \!a_{5k}\right) \!\ge 1, \quad i \!\in \!\{3,5\}, \quad k=\overline{1,M}
	%$$
	\item Since Varnish exhibits load balancing features, it should not be deployed on the same VM as with another type of Balancer (\emph{\textbf{Conflict}} constraint). Moreover, Varnish and MySQL should not be deployed on the same VM because it is best practice to isolate the DBMS level of an application (\emph{\textbf{Conflict}} constraint).
	%$$a_{5 k} + a_{i k} \leq 1, \quad i \in \{2, 3, 4\}, \quad k=\overline{1,M} $$
	\item At least 2 instances of Varnish must be deployed too  (\emph{\textbf{Deployment with bounded number of instances}} constraint, in particular \emph{\textbf{lower bound}}).
	%$$\sum_{k=1}^{M}a_{5k} \ge 2$$
	\item At least 2 different entry points to the MySQL cluster (\emph{\textbf{Deployment with bounded number of instance}} constraint, in particular \emph{\textbf{lower bound}}).
	%$$\sum_{k=1}^{M}a_{2kx} \ge 2$$
	\item No more than 1 DNS server deployed in the administrative domain (\emph{\textbf{Deployment with bounded number of instances}} constraint, in particular \emph{\textbf{upper bound}}).
	%$$\sum_{k=1}^{M}a_{3k} \le 1$$
	\item Balancer components must be placed on a single VM, so they are considered to be in \emph{\textbf{conflict}} with all the other components.
%	\begin{align*}
%	& a_{3 k} + a_{i k} \leq 1 \quad i \in \{1, 2, 5\}\\
%	& a_{4 k} + a_{i k} \leq 1 \quad i \in \{1, 2, 5\} \\
%	\end{align*}
\end{inparaenum}
Depending on the number of Wordpress instaces deployed, SAGE Recommendation Engine outputs two types deployment configurations, one which uses the DNS Load Balancer, the other HTTP Load Balancer (see Tables \ref{tab:Wordpress3SAGE} and \ref{tab:Wordpress8SAGE}).
\begin{table}[h!]
\centering
\begin{tabular}{|l||*{5}{c|}}\hline
\backslashbox{Pod}{Node}
&\makebox[2em]{N1}&\makebox[1em]{N2}&\makebox[1em]{N3}&\makebox[1em]{N4}&\makebox[1em]{N5}\\\hline\hline
WordPress &   1    &                 &            1     &           1      &\\\hline
MySQL     &   1    &    1            &                  &     &\\\hline
DNS       &        &                 &                  &     & 1\\\hline
HTTP      &&&&&\\\hline
Varnish   &        &                 &             1     &    1 &\\\hline
\end{tabular}
\caption{Optimal placement of pods for Wordpress application with 3 Wordpress instances by SAGE}
\label{tab:Wordpress3SAGE}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{|l||*{9}{c|}}\hline
\backslashbox{Pod}{Node}
&\makebox[2em]{N1}&\makebox[1em]{N2}&\makebox[1em]{N3}&\makebox[1em]{N4}&\makebox[1em]{N5}&\makebox[1em]{N6}&\makebox[1em]{N7}&\makebox[1em]{N8}&\makebox[1em]{N9}\\\hline\hline
WordPress &   1    & 1               &            1     &           1      & 1 &1 &1 &  & 1\\\hline
MySQL     &   1    &                 &            1     &           1      & 1 & & & 1 &\\\hline
DNS       &   1    &                 &            1     &           1      & 1 & & & 1 &\\\hline
HTTP      &   1    &                 &            1     &           1      & 1 & & & ? &\\\hline
Varnish &   1    &                 &            1     &           1      & 1 & & & &\\\hline
\end{tabular}
\caption{TODO: Optimal placement of pods for Wordpress application with 8 Wordpress instances by SAGE}
\label{tab:Wordpress8SAGE}
\end{table}

We used the number of nodes and their characteristics for testing Boreas and K8s. Boreas was able to deploy all instances on these nods on both cases, while K8s failed to deploy the DNS load balancer for Wordpress3, respectivelly the HTTP load balancer for Wordpress8. Explanation???


